Language-Forcing: Advancing Humanoid Loco-Manipulation via Semantic Alignment of Whole-Body World Action Models

World Action Models (WAMs) jointly predict robot actions and future observations. However, their visual prediction objectives do not explicitly distinguish task-relevant transitions from incidental scene changes. For whole-body policies, this distinction matters because task progress depends on coordinated changes in body pose, contact, and object state. We introduce LANGUAGE-FORCING, a training strategy that uses language to emphasize task-relevant changes in the future visual representations of a whole-body WAM. Given paired current and ground- truth short-horizon future frames, a frozen vision-language model assesses task progress and predicts plausible subsequent state changes. We encode these descriptions with a frozen text encoder and align their embeddings with intermediate, action-conditioned future-visual features, complementing the original visual and action prediction objectives. All auxiliary components are used only during training, introducing no additional inference overhead. On HumanoidArena, LANGUAGE-FORCING achieves an average success rate of 79.17%, exceeding the strongest competing policy by 9.46 percentage points and the same WAM without language alignment by 10.77 percentage points. Across five real-world tasks, language alignment raises average success from 53.33% to 71.33% over the same WAM baseline.

==> tables/ablation_alignment_depth.tex <==
\begin{wraptable}[11]{r}{0.30\textwidth}
    \centering
    \small
    \setlength{\abovecaptionskip}{2pt}
    \setlength{\belowcaptionskip}{4pt}
    \caption{Alignment depth ablation. SR (\%).}
    \label{tab:ablation-alignment-depth}
    \setlength{\tabcolsep}{4pt}
    \renewcommand{\arraystretch}{1.05}
    \begin{tabular}{cr}
        \toprule
        Block $\ell$ & SR \\
        \midrule
        1  & 73.99 \\
        8  & 74.23 \\
        15 & 75.48 \\
        22 & \textbf{79.17} \\
        29 & 74.46 \\
        \bottomrule
    \end{tabular}
\end{wraptable}


==> tables/ablation_future_frames.tex <==
% tables/ablation_future_frames.tex
% Requires booktabs and wrapfig.

\begin{wraptable}{r}{0.63\textwidth}
    \centering
    \small
    \setlength{\abovecaptionskip}{2pt}
    \setlength{\belowcaptionskip}{4pt}
    \caption{Future video prediction with fixed language supervision.
    All settings include the current frame and repeat images as needed
    to retain five inputs.}
    \label{tab:ablation-temporal-supervision}

    \setlength{\tabcolsep}{3pt}
    \renewcommand{\arraystretch}{1.06}

    \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}ccr@{}}
        \toprule
        \shortstack{Intermediate\\frames}
        & \shortstack{Final frame\\included}
        & SR (\%) \\
        \midrule
        0 & --  & 65.18 \\
        1 & Yes & 72.98 \\
        3 & Yes & \textbf{79.17} \\
        \bottomrule
    \end{tabular*}
\end{wraptable}

==> tables/ablation_loss_weight.tex <==
\begin{wraptable}[8]{l}{0.30\textwidth}
    \centering
    \small
    \setlength{\abovecaptionskip}{2pt}
    \setlength{\belowcaptionskip}{4pt}
    \caption{Language-loss weight ablation. SR (\%).}
    \label{tab:ablation-loss-weight}
    \setlength{\tabcolsep}{4pt}
    \renewcommand{\arraystretch}{1.05}
    \begin{tabular}{cr}
        \toprule
        $\lambda_{\mathrm{LF}}$ & SR \\
        \midrule
        0   & 68.39 \\
        0.5 & 74.40 \\
        1.0 & \textbf{79.17} \\
        1.5 & 73.39 \\
        2.0 & 68.75 \\
        \bottomrule
    \end{tabular}
\end{wraptable}


==> tables/ablation_supervision.tex <==
% tables/ablation_supervision.tex
% Requires booktabs.

\begin{table}[t]
    \centering
    \small
    \caption{Language supervision on HumanoidArena.
    (a) Comparing alignment targets. Captioning and Language Forcing
    receive the same current and future images as VLM inputs,
    but use different prompts.
    (b) Matching or shuffling the descriptions used by Language Forcing
    within each task.
    The WAM training images remain unchanged across settings.}
    \label{tab:lf-supervision}
    \label{tab:ablation-static-vs-change-language}
    \label{tab:ablation-language-shuffle}

    \setlength{\tabcolsep}{4pt}
    \renewcommand{\arraystretch}{1.06}

    \begin{minipage}[t]{0.59\linewidth}
        \centering
        \textbf{(a) Language targets}\par\smallskip
        \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lr@{}}
            \toprule
            Alignment target & SR (\%) \\
            \midrule
            None                         & 68.39 \\
            Task instruction             & 65.18 \\
            Future-image caption         & 73.57 \\
            Task progress and future states
                                         & \textbf{79.17} \\
            \bottomrule
        \end{tabular*}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.37\linewidth}
        \centering
        \textbf{(b) Language pairing}\par\smallskip
        \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lr@{}}
            \toprule
            Pairing & SR (\%) \\
            \midrule
            Shuffled within task & 63.21 \\
            Matched              & \textbf{79.17} \\
            \bottomrule
        \end{tabular*}
    \end{minipage}
\end{table}
